Layout-aware Webpage Quality Assessment

Identifying high-quality webpages is fundamental for real-world search engines, which can fulfil users' information need with the less cognitive burden. Early studies of \emph{webpage quality assessment} usually design hand-crafted features that may only work on particular categories of webpages (e.g., shopping websites, medical websites). They can hardly be applied to real-world search engines that serve trillions of webpages with various types and purposes. In this paper, we propose a novel layout-aware webpage quality assessment model currently deployed in our search engine. Intuitively, layout is a universal and critical dimension for the quality assessment of different categories of webpages. Based on this, we directly employ the meta-data that describes a webpage, i.e., Document Object Model (DOM) tree, as the input of our model. The DOM tree data unifies the representation of webpages with different categories and purposes and indicates the layout of webpages. To assess webpage quality from complex DOM tree data, we propose a graph neural network (GNN) based method that extracts rich layout-aware information that implies webpage quality in an end-to-end manner. Moreover, we improve the GNN method with an attentive readout function, external web categories and a category-aware sampling method. We conduct rigorous offline and online experiments to show that our proposed solution is effective in real search engines, improving the overall usability and user experience.

==> sections/1_intro.tex <==
\section{Introduction}
Search engine, such as Google and Baidu, plays an important role in fulfilling users' information need. Over the past decades, relevance modeling is the main concern of search engine, dedicated to put the most relevant web contents on top of the ranked results~\cite{zou2021pre,liu2021pre,shen2014learning,yin2016ranking}. However, the very fact that not all relevant contents are useful to users has become an increasingly serious symptom, where relevant webpages with low quality would induces significant cognitive burden on the user. In such cases, useful information is hard to be identified, and the users need to take extra effort to understand the information to be conveyed. To reduce the cognitive burden, measuring the quality of webpages has become a critical concern, which can better benefit users with well-delivered information and improve the overall usability of a search engine. For example, given webpages with comparable relevance, the high-quality webpages should be ranked higher than its competitors.

Nevertheless, webpage quality assessment is a very challenging task in practice~\cite{pleasants2021quality}, due to the complexity and diversity of webpages in the era of web 2.0. Early attempts mainly focus on the definition of webpage quality and adopt various heuristics to formulate discriminative features~\cite{moustakis2004website,hasan2011assessing,caro2005data,gupta2021empirical} (e.g., designing user experience based features~\cite{gupta2021empirical}), where classification algorithms~\cite{gupta2021empirical,caro2007bayesian} are applied subsequently. However, the modern search engines usually face billions of webpages with various categories, where simple hand-crafted features may easily fail on such diverse data, and simple classification algorithms (e.g. Bayesian Networks~\cite{caro2007bayesian}) cannot capture the in-depth information that reveals the webpage quality. Worse still, such type of methods may only work well on a particular category of webpages, e.g., shopping websites~\cite{cebi2013quality}, medical website~\cite{rafe2012qualitative}, web portals~\cite{caro2006defining}, and Wikipedia articles~\cite{hasan2009automatic}, where webpages with different categories might be incomparable as the candidates of the same query. 
% For real search engines that benefits billions of users, there is still a lack novel solutions that can effective assess quality for massive webpages without human-designed features.
For real-world search engines that benefits billions of users, there is still a lack of effective solutions that can assess quality for highly diverse webpages.

% Given a certain piece of content, the quality of a webpage is largely determined by its \emph{content layout}. For example, as shown in Figure xxx, a webpage with clear structure, tidy organization and concentrated delivery of key information is always more preferable than the one who only stack relevant information without present it in a proper way, even though they may contain similar or identical information. Existing studies~\cite{wu2021lampret,zhang2020every} have also justified that the layout is of great significance in understanding textual content, and can even benefits down-stream applications. Nevertheless, none of them studies the problem of quality assessment for webpages. 

% To conduct quality assessment for webpages with different categories and purposes, formulating the common representation. 


Notably, despite the categories and purposes of various webpages, all of them can be represented by Document Object Model (DOM), i.e., a cross-platform and language-independent interface that treats a webpage as a tree structure wherein each node is an object representing a part of the webpage. Figure \ref{fig:dom_tree} shows an toy example of the hierarchical structure of a DOM tree, where each node is an object that contains contents of the webpage, and has different attributes (e.g., type and size). Particularly, the DOM tree of a webpage implies its information layout, i.e., how the contents are organized and presented, which is a critical dimension for quality assessment~\cite{moustakis2004website,caro2006defining}, yet is under-explored by existing studies. It is indisputable that inspecting the structure of DOM tree can help to measure the quality of various categories of webpages in a unified manner. In the meantime, it calls for a novel solution that is free of manual feature engineering to extract discriminative features from DOM tree for the task at hand.

\begin{figure}[t]
	\centering
	\includegraphics[width=1\columnwidth]{pic/dom_tree1.pdf}
	\caption{A toy example that shows the structure of DOM tree.}
	\label{fig:dom_tree}
\end{figure}

Recent advances on deep representation learning~\cite{bengio2013representation,lecun2015deep} have achieved great success on many web applications~\cite{shen2014learning,WebQA21,guo2021semantic}, and also sheds new lights on this task. 
% where feature extraction and down-stream tasks are unified with an end-to-end framework
In recent years, a handful of researches~\cite{zhang2020every,huang2019text,yao2019graph} leverage representation learning to perceive text structure (e.g., word interactions) for down-stream tasks, where Graph Neural Networks~\cite{hamilton2017inductive,gilmer2017neural} are widely adopted. Intuitively, the expressiveness of deep representation learning (e.g., GNNs) is also very promising for webpage quality assessment from complex DOM tree structure. However, different from text structure, the webpage layout represented by DOM tree is more complicated, which usually has hierarchical structure and the nodes usually have rich attributes. Existing methods that designed for text structure usually lack specialized consideration for the problem of quality assessment on DOM tree data, and thus might be unsatisfactory for real-world search engines.
% In recent years, there are a handful of studies~\cite{zhang2020every} employs representation learning to .   

% This calls for solutions that can effectively extract discriminate knowledge from DOM trees that can represent the overall quality of webpages.

In this paper, we design a practical solution for the problem of webpage quality assessment, based on the layout information indicated by DOM tree. To model the complicated structure of DOM trees, we first propose a graph construction method that represent a DOM tree as a layout graph. Subsequently, we employ a graph neural network (GNN), which is expressive to reveal the underlying semantics for the quality assessment task. Moreover, we further improve the GNN via more expressive readout function. Besides, to boost the model performance on diverse categories of webpages, we incorporate external category features and leverages a category-aware data sampling method to jointly train the model. The proposed solution is currently fully deployed in the online ranking system of Baidu Search, and we also present the details of how the solution is deployed.

Overall, our main contributions can be summarized as follows.
\begin{itemize}
    \item We develop the largest application of deep learning for the problem of web quality assessment, which is beneficial for improving the overall user experience and usability of Baidu Search.
    \item Based on the DOM tree structure of webpages, we propose a practical solution to learn the quality information in an end-to-end fashion. Moreover, we improve the GNN-based solution with expressive readout function and loss function, and further incorporate category features to boost the model performance.
    \item We conduct rigorous offline and online experiments before fully deploy the model online. The experimental results show that the proposed solution is effective to be applied in real search engines.
\end{itemize}
% Conventional methods have not explored the structure information of the dom tree, where critical information is lost.
% . Considering the scale and complexity of content structure, many deep learning based approaches have been proposed for 

==> sections/1_introduction.tex <==
\section{Introduction}
Search engine, such as Google and Baidu, plays an important role in fulfilling users' information need. 
Over the past decades, relevance modeling is the main concern of search engine, dedicated to put the most relevant web contents on top of the ranked results~\cite{zou2021pre,liu2021pre,shen2014learning,yin2016ranking}. 
However, relevant webpages with low quality would induces significant cognitive burden on the user, where useful information is hard to be identified, and the users need to take extra effort to understand the information to be conveyed. 
To reduce the cognitive burden, measuring the quality of webpages has become a critical concern, which can better benefit users with well-delivered information and improve the overall usability of a search engine. 
% For example, given webpages with comparable relevance, the high-quality webpages should be ranked higher than its competitors.


Nevertheless, webpage quality assessment is a very challenging task in practice~\cite{pleasants2021quality}, due to the complexity and diversity of webpages in the era of web 2.0. Early attempts mainly focus on the definition of webpage quality and adopt various heuristics to formulate discriminative features~\cite{moustakis2004website,hasan2011assessing,caro2005data,gupta2021empirical} (e.g., designing user experience based features~\cite{gupta2021empirical}), where classification algorithms~\cite{gupta2021empirical,caro2007bayesian} are applied subsequently. However, the modern search engines usually face billions of webpages with various categories, where simple hand-crafted features may easily fail on such diverse data, and simple classification algorithms (e.g. Bayesian Networks~\cite{caro2007bayesian}) cannot capture the in-depth information that reveals the webpage quality. Worse still, such type of methods may only work well on a particular category of webpages, e.g., shopping websites~\cite{cebi2013quality}, medical website~\cite{rafe2012qualitative}, web portals~\cite{caro2006defining}, and Wikipedia articles~\cite{hasan2009automatic}, where webpages with different categories might be incomparable as the candidates of the same query. 
% For real search engines that benefits billions of users, there is still a lack novel solutions that can effective assess quality for massive webpages without human-designed features.
For real-world search engines that benefit billions of users, there is still a lack of effective solutions that can assess quality for highly diverse webpages.


Given a certain piece of content, the quality of a webpage is largely determined by its \emph{content layout}~\cite{moustakis2004website,caro2006defining}. A webpage with clear structure, tidy organization and concentrated delivery of key information is always more preferable than the one who only stack relevant information without present it in a proper way, even though they may contain similar or identical information. 
Existing studies~\cite{wu2021lampret,zhang2020every} have also justified that the layout is of great significance in understanding textual content, and can even benefits down-stream applications. Nevertheless, none of them studies the problem of quality assessment for webpages. 


Notably, despite the categories and purposes of various webpages, all of them can be represented by Document Object Model (DOM), i.e., a cross-platform and language-independent interface that treats a webpage as a tree structure wherein each node is an object representing a part of the webpage. Figure \ref{fig:dom_tree} shows an toy example of the hierarchical structure of a DOM tree, where each node is an object that contains contents of the webpage, and has different attributes (e.g., type and size). Particularly, the DOM tree of a webpage implies its information layout, i.e., how the contents are organized and presented, which is a critical dimension for quality assessment~\cite{moustakis2004website,caro2006defining}, yet is under-explored by existing studies. It is indisputable that inspecting the structure of DOM tree can help to measure the quality of various categories of webpages in a unified manner. In the meantime, it calls for a novel solution that is free of manual feature engineering to extract discriminative features from DOM tree for the task at hand.

\begin{figure}[t]
	\centering
	\includegraphics[width=1\columnwidth]{pic/dom_tree1.pdf}
	\caption{A toy example that shows the structure of DOM tree.}
	\label{fig:dom_tree}
\end{figure}

Recent advances on deep representation learning~\cite{bengio2013representation,lecun2015deep} have achieved great success on many web applications~\cite{shen2014learning,Chang2021WebQAMA,guo2021semantic}, and also sheds new lights on this task. 
% where feature extraction and down-stream tasks are unified with an end-to-end framework
In recent years, a handful of researches~\cite{zhang2020every,huang2019text,yao2019graph} leverage representation learning to perceive text structure (e.g., word interactions) for down-stream tasks, where Graph Neural Networks~\cite{hamilton2017inductive,gilmer2017neural} are widely adopted. Intuitively, the expressiveness of deep representation learning (e.g., GNNs) is also very promising for webpage quality assessment from complex DOM tree structure. However, different from text structure, the webpage layout represented by DOM tree is more complicated, which usually has hierarchical structure and the nodes usually have rich attributes. Existing methods that designed for text structure usually lack specialized consideration for the problem of quality assessment on DOM tree data, and thus might be unsatisfactory for real search engines.

In this paper, we design a practical solution for the problem of webpage quality assessment, based on the layout information indicated by DOM tree. To model the complicated structure of DOM trees, we first propose a graph construction method that represent a DOM tree as a layout graph. Subsequently, we employ a graph neural network (GNN), which is expressive to reveal the underlying semantics for the quality assessment task. Moreover, we further improve the GNN via more expressive readout function. Besides, to boost the model performance on diverse categories of webpages, we incorporate external category features and leverages a category-aware data sampling method to jointly train the model. The proposed solution is currently fully deployed in the online ranking system of Baidu Search, and we also present the details of how the solution is deployed.
Overall, our main contributions can be summarized as follows.
\begin{itemize}
    \item We develop the largest application of deep learning for the problem of layout-aware web quality assessment, which is beneficial for improving the overall user experience and usability of Baidu Search.
    \item Based on the layout structure of webpages (the DOM tree), we propose a practical solution to learn the quality information in an end-to-end fashion. Moreover, we improve the GNN-based solution with an expressive readout function and a loss function, and further incorporate category features to boost the model performance.
    \item We conduct rigorous offline and online experiments before fully deploy the model online. The experimental results show that the proposed solution is effective to be applied in the real-world search engines.
\end{itemize}
% Conventional methods have not explored the structure information of the dom tree, where critical information is lost.
% . Considering the scale and complexity of content structure, many deep learning based approaches have been proposed for 

==> sections/2_related_work.tex <==
\section{Related Work}
\subsection{Graph Neural Network}
Recent years have witnessed the success of graph neural networks (GNNs) for relational data. 
For example, Graph Convolutional Network (GCN) \cite{Kipf2017SemiSupervisedCW} is introduced to aggregate the one-hop neighbours of each node in the graph, followed by a linear projection and non-linear activation. 
GraphSAGE \cite{hamilton2017inductive} is proposed to generalize GCN’s aggregation operation from average to sum, max and a RNN unit. 
Graph Attention Network (GAT) \cite{velivckovic2017graph} employs the attention mechanism into GNNs, which allows GAT to assign different importance to nodes within the same neighbourhood.
Generally, a GNN can be regarded as using the input graph structure as the computation graph for message passing~\cite{gilmer2017neural}, during which the local neighbourhood information is aggregated to get a more contextual representation. 
For more details, please refer to \cite{wu2020comprehensive}. 

% GNN Useful Applications
Moreover, there are many applications across various domains that apply GNNs and achieve considerable improvements, such as protein model quality assessment \cite{Sanyal2020ProteinGCNPM,Baldassarre2021GraphQAPM}, fuel ignition quality assessment \cite{Schweidtmann2020GraphNN}, advertising detection \cite{Yang2022WTAGRAPHWT} and text classification \cite{yao2019graph,Huang2019TextLG,Ding2020BeMW,zhang2020every}. 
For example, Sanyal et al. \cite{Sanyal2020ProteinGCNPM} explore an alternative approach and train a graph convolutional network with nodes representing protein atoms and edges connecting spatially adjacent atom pairs.
GraphQA \cite{Baldassarre2021GraphQAPM} is a graph-based method to estimate the quality of protein models, that possesses favorable properties such as representation learning.
Schweidtmann et al. \cite{Schweidtmann2020GraphNN} develop GNN models for predicting three fuel ignition quality indicators of oxygenated and non-oxygenated hydrocarbons.
Yang et al. \cite{Yang2022WTAGRAPHWT} propose WTAGRAPH, a web tracking and advertising detection framework based on graph neural networks.

Notably, a handful of researches~\cite{zhang2020every,huang2019text,yao2019graph} leverage GNN to perceive text structure (e.g., word interactions) for down-stream tasks, which are the closest research to our study. However, they mainly consider the relationships between segments of text (e.g., words and paragraphs), and do not consider the overall structure and layout of webpage, i.e., how the multi-modal content is organized and presented. In addition, the expressiveness of GNN is not explored for the task of webpage quality assessment. In this paper, we develop the first GNN-based method for webpage quality assessment, which is further deployed in the real production environment that facilitate the usability of our search engine.

% Difference
% The key difference between our approach and existing attempts is that we construct the graph of webpage based on layout for improved webpage quality assessment.

\subsection{Layout}
% Layout is one key dimension for webpage quality
Layout, i.e., how the contents are organized and presented, is a critical dimension for document generation \cite{Biswas2021GraphbasedDG}, scene recognition \cite{Avetisyan2020SceneCADPO,Chen2020SceneRW} and webpage quality assessment \cite{moustakis2004website,hasan2011assessing}.
Substantial efforts have been made to explore the importance of layout in many AI areas. 
For example, Besides, Biswas et al. \cite{Biswas2021GraphbasedDG} design an automated deep generative model using graph neural networks to generate synthetic data with highly variable and plausible document layouts.
% For scene recognition areas,
Avetisyan et al. \cite{Avetisyan2020SceneCADPO} use a message-passing graph neural network to model the inter-relationships between objects and layout, guiding the generation of a global object alignment in a scene. 
Chen et al. \cite{Chen2020SceneRW} build a Layout Graph Network (LGN) where regions in PaSL are defined as nodes and two kinds of independent relations between regions are encoded as edges. 
Zhang et al. \cite{Zhang2021LithographyLC} propose a new kind of classification method for lithography layout patterns based on graph convolution network.

Recently, with the development of pre-trained language models, LayoutLM-style methods have achieved success in textual or multi-model document understanding.
For instance,
LAMPreT~\cite{wu2021lampret} encodes each block with a multimodal transformer in the lower-level, and aggregates the block-level representations and connections utilizing a specifically designed transformer at the higher-level.
LayoutLM~\cite{Xu2020LayoutLMPO} jointly model interactions between text and layout information across scanned document images, which is beneficial for a great number of real-world document image understanding tasks such as information extraction from scanned documents.
LayoutLM-v2 \cite{Xu2021LayoutLMv2MP} further uses the new text-image alignment and text-image matching tasks and integrates a spatial-aware self-attention mechanism into the Transformer architecture.
LayoutLM-v3 \cite{Huang2022LayoutLMv3PF} pre-trains multi-modal Transformers for Document AI with unified text and image masking.

Our work differs from the aforementioned studies, as our main focus is to model the layout of webpages for quality assessment. In particular, we model the layout of webpage with a graph construction method that represents a DOM tree as a layout graph and employ an expressive graph neural network to capture the underlying semantics of the layout graphs for webpage quality assessment.

